PerceMon: Online Monitoring for Perception Systems

Perception algorithms in autonomous vehicles are vital for the vehicle to understand the semantics of its surroundings, including detection and tracking of objects in the environment. The outputs of these algorithms are in turn used for decision-making in safety-critical scenarios like collision avoidance, and automated emergency braking. Thus, it is crucial to monitor such perception systems at runtime. However, due to the high-level, complex representations of the outputs of perception systems, it is a challenge to test and verify these systems, especially at runtime. In this paper, we present a runtime monitoring tool, PerceMon that can monitor arbitrary specifications in Timed Quality Temporal Logic (TQTL) and its extensions with spatial operators. We integrate the tool with the CARLA autonomous vehicle simulation environment and the ROS middleware platform while monitoring properties on state-of-the-art object detection and tracking algorithms.

==> sections/monitor.tex <==



==> sections/past-time.tex <==
To define the past-time syntax and semantics for STQL, we use notation similar
to~\cite{maler_real_2005,maler_mitl_2006,maler_synthesizing_2007}.

\begin{definition}[Past-time STQL]
  Let \(V_x, V_f, V_o\) be sets of time variables, frame variables, and object
  ID variables respectively. Then, the syntax for the past-time formalization
  of STQL is as follows:
  \begin{align*}
    % Top-level expression
    \Phi ::=\quad%
     & \exists\{ id_1, id_2, \ldots\}@\{x, f\}.\Phi                                           % Pin frame and id
    \mid \exists\{ id_1, id_2, \ldots\}.\Phi          % Pin only id
    \mid \{x,f\}.\Phi                     % Pin only frame
    \\
     & \mid \top \mid \neg\Phi \mid \Phi \lor \Phi \mid \Prev\Phi \mid \Phi \Since \Phi       \\
     & \mid x - \CTIME \sim t \mid f - \CFRAME \sim n                                         \\
     & \mid \idcls(id_i) = c \mid \idcls(id_i) = \idcls(id_i)
    \mid \idprob(id_i) \sim r \mid \idprob(id_i) \sim r \times \idprob(id_j)                  \\
     & \mid \{id_i = id_j\} \mid \{id_i \not= id_j\} \mid \SpExists \Omega \mid \Pi
    \\ % Topological operations
    \Omega ::=\quad
     & \varnothing \mid \Universal \mid \BBox(id_1)
    \mid \Comp\Omega \mid \Omega \sqcup \Omega \mid \Interior \Omega                          \\
     & \mid \SpPrev \Omega \mid \SpAlwP \Omega \mid \SpEvP \Omega \mid \Omega \SpSince \Omega
    \\ % Area operations
    \Pi ::=\quad
     & \Area(\Omega) \sim r | \Area(\Omega) \sim r \times \Area(\Omega)                       \\
     & \mid \ED(id_i, \CRT, id_j, \CRT) \sim r
    \mid \Theta \sim r \mid \Theta \sim r \times \Theta
    \\ % Distance operations
    \Theta ::=\quad
     & \Lat(id_i, \CRT) \mid \Lon(id_i, \CRT)
    \\ % Reference points
    \CRT ::=\quad
     & \LM \mid \RM \mid \TM \mid \BM \mid \CT
  \end{align*}
  where, \(x \in V_x, f \in V_f\), and \(id_i, id_j \in V_o \).
\end{definition}

The time and frame constraints of Past-STQL are represented in the form \(x -
\CTIME\) and \(f - \CFRAME\), as in the case of past-time operators, \(x \geq
\CTIME, f \geq \CFRAME\).
Here, we also introduce the following \emph{past-time} temporal operators:
\begin{enumerate}
  \item \emph{Previous}, \(\Prev \varphi\) (the past-time counterpart for the Next \(\Next\));
  \item \emph{Since}, \(\varphi \Since \varphi\) (the past-time counterpart for the Until \(\Unt\));
  \item \emph{Back To}, \(\varphi \Back \varphi\) (counterpart for Release \(\Release\));
  \item \emph{Once} in the past, \(\EvP \varphi\);
  \item \emph{Holds} in the past, \(\AlwP \varphi\);
\end{enumerate}


\begin{definition}[Past-time STQL Semantics]
  Consider a data stream \(\xi\) consisting of \emph{frames} containing objects and
  annotated with a time stamp. Let \(i \in \Naturals\) be the current frame of
  evaluation, and let \(\xi_i\) denote the \(i^{th}\) frame. We let \(\epsilon: V_t \cup
  V_f \to \Naturals \cup \{\NaN\} \) denote a mapping from a pinned time or frame
  variable to a frame index (if it exists), and let \(\zeta: V_o \to \Naturals\) be a
  mapping from an object variable to an actual object ID that was assigned by a
  quantifier. Finally, we let \(\Oc(\xi_i)\) denote the set of object IDs available in
  the frame \(i\), and let \(t(\xi_i)\) output the timestamp of the given frame.

  Let \(\Quality{\varphi}\) be the quality of the \paststql{} formula, \(\varphi\), at
  the current frame \(i\), which can be recursively defined as follows:
  \begin{align*}
    \Quality{\top}(\xi, i, \epsilon, \zeta)         & = \top                                                                                                                                              \\
    \Quality{\exists\{id_1,\ldots,id_n\} @ {x,f} . \phi}(\xi, i, \epsilon, \zeta)
                                                    & = \bigvee_{k_1,\ldots,k_n \in \Oc(\xi_i)}\left(\Quality{\phi}(\xi, i, \epsilon[x \gets t(\xi_i), f \gets i], \zeta[id_1 \gets k_1, \ldots]  \right) \\
    \Quality{x - \CTIME \sim c}(\xi, i, \epsilon, \zeta)
                                                    & = \begin{cases}
      \top,\quad\text{if } \epsilon(x) - t(\xi_i) \sim c \\
      \bot,\quad\text{otherwise.}
    \end{cases}                                                                                                                         \\
    \Quality{f - \CFRAME \sim c}(\xi, i, \epsilon, \zeta)
                                                    & = \begin{cases}
      \top,\quad\text{if } \epsilon(f) - i \sim c \\
      \bot,\quad\text{otherwise.}
    \end{cases}                                                                                                                         \\
    \Quality{\{id_j = id_j\}}(\xi, i, \epsilon, \zeta)
                                                    & = \begin{cases}
      \top,\quad\text{if } \zeta(id_j) = \zeta(id_k) \\
      \bot,\quad\text{otherwise.}
    \end{cases}                                                                                                                         \\
    \Quality{\idcls(id_j) = c}(\xi, i, \epsilon, \zeta)
                                                    & = \begin{cases}
      \top,\quad\text{if } \Oc(\xi_i)(\zeta(id_j)).\textrm{class} = c \\
      \bot,\quad\text{otherwise.}
    \end{cases}                                                                                                                         \\
    \Quality{\idcls(id_j) = \idcls(id_k)}(\xi, i, \epsilon, \zeta)
                                                    & = \begin{cases}
      \top,\quad\text{if } \Oc(\xi_i)(\zeta(id_j)).\textrm{class} = \Oc(\xi_i)(\zeta(id_k)).\textrm{class} \\
      \bot,\quad\text{otherwise.}
    \end{cases}                                                                                                                         \\
    \Quality{\idprob(id_j) \sim r}(\xi, i, \epsilon, \zeta)
                                                    & = \begin{cases}
      \top,\quad\text{if } \Oc(\xi_i)(\zeta(id_j)).\textrm{prob} \sim r \\
      \bot,\quad\text{otherwise.}
    \end{cases}                                                                                                                         \\
    \Quality{\idprob(id_j) \sim r \times \idprob(id_k)}(\xi, i, \epsilon, \zeta)
                                                    & = \begin{cases}
      \top,\quad\text{if } \Oc(\xi_i)(\zeta(id_j)).\textrm{prob} \sim r \times \Oc(\xi_i)(\zeta(id_k)).\textrm{prob} \\
      \bot,\quad\text{otherwise.}
    \end{cases}                                                                                                                         \\
    \Quality{\neg\varphi}(\xi, i, \epsilon, \zeta)  & = \neg\Quality{\varphi}(\xi, i, \epsilon, \zeta)                                                                                                    \\
    \Quality{\varphi_1 \lor \varphi_2}(\xi, i, \epsilon, \zeta)
                                                    & = \Quality{\varphi_i}(\xi, i, \epsilon, \zeta) \lor \Quality{\varphi_2}(\xi, i, \epsilon, \zeta)                                                    \\
    \Quality{\Prev\varphi}(\xi, i, \epsilon, \zeta) & = \Quality{\Prev\varphi}(\xi, i - 1, \epsilon, \zeta)                                                                                               \\
    \Quality{\varphi_1 \Since \varphi_2}(\xi, i, \epsilon, \zeta)
                                                    & = \bigvee_{j \leq i}\left(
    \Quality{\varphi_2}(\xi, j, \epsilon, \zeta) \land \bigwedge_{j \leq k \leq i} \Quality{\varphi_1}(\xi, k, \epsilon, \zeta)
    \right)                                                                                                                                                                                               \\
    \Quality{\SpExists\Tc}(\xi, i, \epsilon, \zeta)
                                                    & = \begin{cases}
      \top,\quad\text{if } \SpEval(\Tc, \xi, i, \epsilon, \zeta) \not= \emptyset \\
      \bot,\quad\text{otherwise.}
    \end{cases}                                                                                                                        \\
    \Quality{\Area(\Tc_1) \sim r}
                                                    & = \begin{cases}
      \top,\quad\text{if } \Area(\SpEval(\Tc_1, \xi, i, \epsilon, \zeta)) \sim r \\
      \bot,\quad\text{otherwise.}
    \end{cases}                                                                                                                        \\
    \Quality{\Lat(id_1, \CRT_1) \sim r}(\xi, i, \epsilon, \zeta)
                                                    & = \begin{cases}
      \top,\quad\text{if } f_{lat}{}(id_1, \CRT_1, \xi, i, \epsilon, \zeta) \sim r \\
      \bot,\quad\text{otherwise.}
    \end{cases}                                                                                                                        \\
    \Quality{\Lon(id_1, \CRT_1) \sim r}(\xi, i, \epsilon, \zeta)
                                                    & = \begin{cases}
      \top,\quad\text{if } f_{lon}(id_1, \CRT_1, \xi, i, \epsilon, \zeta) \sim r \\
      \bot,\quad\text{otherwise.}
    \end{cases}
  \end{align*}
  where, \(\sim \in \Set{<,>,\leq,\geq}\), and the operations \(\SpEval\), \(f_{lon}\), and \(f_{lat}\) are defined as follows:
  \begin{enumerate}
    \item \(f_{lat}\) computes the \emph{lateral distance} of the \(\CRT\) point of an object identified by \(\Oc(\zeta(id_1))\) from the \emph{Longitudnal axis}.
    \item \(f_{lon}\) computes the \emph{longitudnal distance} of the \(\CRT\) point of an object identified by \(\Oc(\zeta(id_1))\) from the \emph{Lateral axis}.
    \item \(\SpEval(\Tc, \xi, i, \epsilon, \zeta)\) is the set operations over bounding
          boxes with temporal modalities. Due to space restrictions, and the overlapping
          definitions with existing operators, we forgo from explictely defining this.
          % \needtowrite{Appendix: Spatial semantics.}
  \end{enumerate}

\end{definition}

On a high-level, the semantics for the past-time temporal operators is
equivalent to interpreting their forward-time counterparts over a reversed data
stream/signal. This implies that, for a signal \(\xi\) and a Past-STQL formula
\(\varphi\) evaluated at time \(t\), if the reversed signal \(\xi' = (\xi_t,
\ldots, \xi_0)\) is such that \((\xi', t) \models \varphi'\), where \(\varphi'\)
is the given formula with all past-time temporal operators replaced with their
equivalent forward-time counterparts, then \((\xi, t)\models \varphi\).

\begin{definition}[Monitoring Horizon]\label{def:horizon}
  For a \paststql{} formula \(\varphi\) and a signal/data stream \(\xi\)
  evaluated at time \(t\), the \emph{monitoring horizon}, \(\Horizon(\varphi)\)
  is the maximum length of signal required to correctly compute
  whether \((\xi, t) \models \varphi\).
  \begin{align*}
          & \Horizon(\neg \varphi)             & =\quad & \Horizon(\varphi)                                  \\
          & \Horizon(\varphi_1 \lor \varphi_2) & =\quad & \max\of*{\Horizon(\varphi_1), \Horizon(\varphi_2)} \\
          & \Horizon(\Prev \varphi)            & =\quad & 1 + \Horizon(\varphi)                              \\
          & \Horizon(\EvP \varphi)             & =
    \quad &
    \begin{cases}
      c + \Horizon(\psi)\qquad\text{when, } \varphi \equiv (f - \CFRAME < c) \land \psi \\
      \infty\qquad\qquad\quad~\text{otherwise.}
    \end{cases}                                                                               \\
          & \Horizon(\AlwP\varphi)             & =
    \quad &
    \begin{cases}
      c + \Horizon(\psi)\qquad\text{when, } \varphi \equiv (f - \CFRAME < c) \implies \psi \\
      \infty\qquad\qquad\quad~\text{otherwise.}
    \end{cases}                                                                               \\
          & \Horizon\varphi_1 \Since \varphi_2 & =
    \quad &
    \begin{cases}
      c + \max\of*{\Horizon(\varphi_1), \Horizon(\psi)} \text{when, } \varphi_2 \equiv (f - \CFRAME < c) \implies \psi \\
      \infty\qquad\qquad\quad~\text{otherwise.}
    \end{cases}                                                                               \\
          & \Horizon\of{\varphi}               & =\quad & 0, \quad\text{otherwise.}
  \end{align*}
\end{definition}







==> sections/results.tex <==
In this section, we are going to demonstrate some results from online monitoring of real
world multi-object tracking algorithms. We use the algorithm presented
in~\cite{zhang_simple_2020} to track pedestrians in videos given in the MOT17
benchmarking dataset~\cite{milan_mot16_2016}, and output a stream of frames. The
perception algorithm classifies a detected object as a \emph{pedestrian} or doesn't
classify it as anything at all. It also assigns to each detected object a unique ID (as
a number in \(\Naturals\)), a confidence level (normalized between 0 and 1), and a
bounding box that surrounds the object.

In the following demonstrations, we focus on requirements that check some ``common
sense'' properties imposed on perception systems. Specifically, we check for persistent
detection and potential occlusions.

\subsection{Example 1: Persistent Detection}%
\label{sub:example1}

In this example, we are interested in monitoring the following high-level specification:
\begin{displayquote}
  If an object is detected in the current image with high confidence and away from the
  margins, then it must have been present in the previous set of frames too.
\end{displayquote}
In this specification, we are essentially interested in tracking is there is a span of
time when we lose track of an object that is in the current frame. Formally, the
specification is as follows:
\begin{align}
  \begin{split}
    \phi &:= \forall\Set{id_1} @ \Set{f}.\left( \left(\phi_{\text{high prob}} \land \phi_{\text{margins}}\right) \Rightarrow \Alw\phi_{\text{exists}}\right) \\[1em]
    \phi_{\text{high prob}} &:= \idprob(id_1) > 0.8 \land\idcls(id_1) = \textsf{PED} \\
    \phi_{\text{margins}} &:= \Lon(id_1, \TM) > c_1 \land \Lon(id_1, \BM) < c_2 \\
    &\quad\land \Lat(id_1, \LM) > c_3 \land \Lat(id_1, \RM) < c_4 \\
    \phi_{\text{exists}} &:= (f - \CFRAME < 6) \\
    &\quad \Rightarrow \exists\{id_2\}.\left(\{id_1 = id_2\} \land \idprob(id_2) > 0.7 \land \idcls(id_2) = \textsf{PED}\right)
  \end{split}
\end{align}

\begin{figure}
  \centering
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example1/00022.jpg}
    \caption{Frame 22.}
  \end{subfigure}
  ~%
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example1/00023.jpg}
    \caption{Frame 23.}
  \end{subfigure}
  ~%
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example1/00024.jpg}
    \caption{Frame 24.}
  \end{subfigure}
  ~%
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example1/00025.jpg}
    \caption{Frame 25.}
  \end{subfigure}
  ~%
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example1/00026.jpg}
    \caption{Frame 26.}
  \end{subfigure}
  ~%
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example1/00027.jpg}
    \caption{Frame 27.}
  \end{subfigure}

  \caption{A snippet from the video \texttt{MOT17--03}. Here, it can be seen that the
  bounding boxes around the pedestrians in the frame are being lost. The perception
  monitor is able to detect these lost frames.}%
\end{figure}


\subsection{Example 2: Potential Occlusions}%
\label{sub:example1}

In this example, we are interested in monitoring the following high-level specification:
\begin{displayquote}
  If an object is detected in the current image with high confidence and away from the
  margins, it should not have been overlapping with another object too much.
\end{displayquote}
In this specification, we are essentially interested in checking if any object was too
close to another object, and could have potentially occluded the other object. Formally,
the specification is as follows:
\begin{align}
  \begin{split}
   \phi &:= \forall\Set{id_1} @ \Set{x}.\left( \left(\phi_{\text{high prob}} \land \phi_{\text{margins}}\right)\right. \\
   &\qquad\qquad\qquad\left. \Rightarrow \Alw(x - \CTIME < 1.0 \Rightarrow \neg\phi_{\text{occluding}}\right) \\[1em]
   \phi_{\text{high prob}} &:= \idprob(id_1) > 0.8 \\
   \phi_{\text{margins}} &:= \Lon(id_1, \TM) > c_1 \land \Lon(id_1, \BM) < c_2 \\
                         &\quad\land \Lat(id_1, \LM) > c_3 \land \Lat(id_1, \RM) < c_4 \\
   \phi_{\text{occluding}} &:=\exists\{id_2\}.\left(\{id_1 = id_2\} \land \idprob(id_2) > 0.7\right.\\
   &\quad\left.\land \forall\{id_3\} . \right(\{id_3 \not= id_2\} \Rightarrow (\Area(\BBox(id_3) \sqcap \BBox(id_2)) > a_1) \left)\right)
  \end{split}
\end{align}

\begin{figure}
  \centering
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example2/00122.jpg}
    \caption{Frame 122.}
  \end{subfigure}
  ~%
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example2/00123.jpg}
    \caption{Frame 123.}
  \end{subfigure}
  ~%
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example2/00124.jpg}
    \caption{Frame 124.}
  \end{subfigure}
  ~%
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example2/00125.jpg}
    \caption{Frame 125.}
  \end{subfigure}
  ~%
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example2/00126.jpg}
    \caption{Frame 126.}
  \end{subfigure}
  ~%
  \begin{subfigure}[t]{0.15\textwidth}
    \centering
    \includegraphics[height=2cm,keepaspectratio]{imgs/Example2/00127.jpg}
    \caption{Frame 127.}
  \end{subfigure}

  \caption{A snippet from the video \texttt{MOT17--03}. Here, it can be seen that the
  bounding boxes around the pedestrians in the frame are being lost due to various
  reasons, including occlusions. Our perception monitor is able to detect these
  occlusions before it happens.}%
\end{figure}




==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_EXCMD	mixed	/number, pattern, mixed, or combineV2/
!_TAG_OUTPUT_FILESEP	slash	/slash or backslash/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PATTERN_LENGTH_LIMIT	96	/0 for no limit/
!_TAG_PROC_CWD	/home/anand/workspace/writing/rv2021/	//
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	5.9.0	/b537b4ff/
-0,0 +1,146	diff-since-submission.diff	/^@@ -0,0 +1,146 @@$/;"	h	newFile:b/main.tex
-1,12 +1,12	diff-since-submission.diff	/^@@ -1,12 +1,12 @@$/;"	h	modifiedFile:a/sections/intro.tex
-1,3 +1,5	diff-since-submission.diff	/^@@ -1,3 +1,5 @@$/;"	h	modifiedFile:a/sections/appendix.tex
-1,4 +1,4	diff-since-submission.diff	/^@@ -1,4 +1,4 @@$/;"	h	modifiedFile:a/sections/stql.tex
-1,7 +1,13	diff-since-submission.diff	/^@@ -1,7 +1,13 @@$/;"	h	modifiedFile:a/sections/percemon.tex
-1,93 +1,111	diff-since-submission.diff	/^@@ -1,93 +1,111 @@$/;"	h	modifiedFile:a/sections/experiments.tex
-14,12 +20,11	diff-since-submission.diff	/^@@ -14,12 +20,11 @@$/;"	h	modifiedFile:a/sections/percemon.tex
-18,31 +18,34	diff-since-submission.diff	/^@@ -18,31 +18,34 @@$/;"	h	modifiedFile:a/sections/intro.tex
-27,7 +32,9	diff-since-submission.diff	/^@@ -27,7 +32,9 @@ \\subsection{Integration with CARLA and ROS}%$/;"	h	modifiedFile:a/sections/percemon.tex
-47,61 +47,109	diff-since-submission.diff	/^@@ -47,61 +47,109 @@$/;"	h	modifiedFile:a/sections/stql.tex
-52,3 +59,11	diff-since-submission.diff	/^@@ -52,3 +59,11 @@ \\subsection{Integration with CARLA and ROS}%$/;"	h	modifiedFile:a/sections/percemon.tex
400568	bib.bib	/^@article{400568,$/;"	a
8237586	bib.bib	/^@inproceedings{8237586,$/;"	j
9078755	bib.bib	/^@article{9078755,$/;"	a
Acknowledgment	main.tex	/^\\section*{Acknowledgment}$/;"	s
Conclusion	main.tex	/^\\section{Conclusion}%$/;"	s
Consistent Detections $\\varphi_1$	sections/experiments.tex	/^\\paragraph{Consistent Detections $\\varphi_1$}: For all objects in the current frame$/;"	P	section:Semantics for STQL
Example 1: Persistent Detection	sections/results.tex	/^\\subsection{Example 1: Persistent Detection}%$/;"	u	section:Semantics for STQL
Example 2: Potential Occlusions	sections/results.tex	/^\\subsection{Example 2: Potential Occlusions}%$/;"	u	section:Semantics for STQL
Experiments	main.tex	/^\\section{Experiments}%$/;"	s
Integration with CARLA and ROS	sections/percemon.tex	/^\\subsection{Integration with CARLA and ROS}%$/;"	u	section:Semantics for STQL
Introduction	main.tex	/^\\section{Introduction}%$/;"	s
PerceMon: An Online Monitoring Tool	main.tex	/^\\section{PerceMon: An Online Monitoring Tool}%$/;"	s
Related work	sections/intro.tex	/^\\paragraph{Related work}%$/;"	P	section:Semantics for STQL
Semantics for STQL	sections/appendix.tex	/^\\section{Semantics for STQL}%$/;"	s
Smooth Object Trajectories $\\varphi_2$	sections/experiments.tex	/^\\paragraph{Smooth Object Trajectories $\\varphi_2$}: For every object in the current$/;"	P	section:Semantics for STQL
Spatio-temporal Quality Logic	main.tex	/^\\section{Spatio-temporal Quality Logic}%$/;"	s
\\@startsection{paragraph}{4}{\\z@} {-12\\p@ \\@plus -4\\p@ \\@minus -4\\p@} {-0.5em \\@plus -0.22em \\@minus -0.1em} {\\normalfont\\normalsize\\bfseries}	main.tex	/^\\renewcommand\\paragraph{\\@startsection{paragraph}{4}{\\z@}%$/;"	P
\\algorithmautorefname	main.tex	/^\\newcommand{\\algorithmautorefname}{Algorithm}$/;"	C
\\cmark	main.tex	/^\\newcommand{\\cmark}{\\ding{51}}%$/;"	C
\\definitionautorefname	main.tex	/^\\newcommand{\\definitionautorefname}{Definition}$/;"	C
\\done	main.tex	/^\\newcommand{\\done}{\\rlap{$\\square$}{\\raisebox{2pt}{\\large\\hspace{1pt}\\cmark}}%$/;"	C
\\refappendix	main.tex	/^\\newcommand{\\refappendix}[1]{\\hyperref[#1]{Appendix~\\ref*{#1}}}$/;"	C
\\todo	main.tex	/^\\newcommand{\\todo}[1]{\\textcolor{red}{#1}}$/;"	C
\\wontfix	main.tex	/^\\newcommand{\\wontfix}{\\rlap{$\\square$}{\\large\\hspace{1pt}\\xmark}}$/;"	C
\\xmark	main.tex	/^\\newcommand{\\xmark}{\\ding{55}}%$/;"	C
a/sections/appendix.tex	diff-since-submission.diff	/^--- a\/sections\/appendix.tex$/;"	m
a/sections/experiments.tex	diff-since-submission.diff	/^--- a\/sections\/experiments.tex$/;"	m
a/sections/intro.tex	diff-since-submission.diff	/^--- a\/sections\/intro.tex$/;"	m
a/sections/percemon.tex	diff-since-submission.diff	/^--- a\/sections\/percemon.tex$/;"	m
a/sections/stql.tex	diff-since-submission.diff	/^--- a\/sections\/stql.tex$/;"	m
annpureddy_staliro_2011	bib.bib	/^@incollection{annpureddy_staliro_2011,$/;"	I
antonante_monitoring_2020	bib.bib	/^@article{antonante_monitoring_2020,$/;"	a
b/main.tex	diff-since-submission.diff	/^+++ b\/main.tex$/;"	n
balakrishnan_specifying_2019	bib.bib	/^@inproceedings{balakrishnan_specifying_2019,$/;"	j
bartocci_specificationbased_2018	bib.bib	/^@incollection{bartocci_specificationbased_2018,$/;"	I
bauer_decentralised_2012	bib.bib	/^@inproceedings{bauer_decentralised_2012,$/;"	j
bernardin_evaluating_2008	bib.bib	/^@article{bernardin_evaluating_2008,$/;"	a
bortolussi_specifying_2014	bib.bib	/^@inproceedings{bortolussi_specifying_2014,$/;"	j
bouyer_expressiveness_2005	bib.bib	/^@incollection{bouyer_expressiveness_2005,$/;"	I
darknet13	bib.bib	/^@misc{darknet13,$/;"	n
def:horizon	sections/past-time.tex	/^\\begin{definition}[Monitoring Horizon]\\label{def:horizon}$/;"	l
def:stql-syntax	sections/stql.tex	/^  \\label{def:stql-syntax} Let \\(V_t\\) be a set of time variables, \\(V_f\\) be a set of$/;"	l
deshmukh_robust_2017	bib.bib	/^@article{deshmukh_robust_2017,$/;"	a
dokhanchi_evaluating_2018	bib.bib	/^@inproceedings{dokhanchi_evaluating_2018,$/;"	j
dokhanchi_online_2014	bib.bib	/^@inproceedings{dokhanchi_online_2014,$/;"	j
donze_automotive_2015	bib.bib	/^@inproceedings{donze_automotive_2015,$/;"	j
donze_efficient_2013	bib.bib	/^@inproceedings{donze_efficient_2013,$/;"	j
donze_robust_2010	bib.bib	/^@inproceedings{donze_robust_2010,$/;"	j
dosovitskiy_carla_2017	bib.bib	/^@inproceedings{dosovitskiy_carla_2017,$/;"	j
dreossi_verifai_2019	bib.bib	/^@incollection{dreossi_verifai_2019,$/;"	I
everingham_pascal_2015	bib.bib	/^@article{everingham_pascal_2015,$/;"	a
fainekos_robustness_2009	bib.bib	/^@article{fainekos_robustness_2009,$/;"	a
fainekos_robustness_2019	bib.bib	/^@incollection{fainekos_robustness_2019,$/;"	I
falanga_vision-based_2017	bib.bib	/^@inproceedings{falanga_vision-based_2017,$/;"	j
fig:carla-experiments	sections/experiments.tex	/^  \\label{fig:carla-experiments}%$/;"	l
fig:pedestrian-crossing-scenario	sections/experiments.tex	/^    \\label{fig:pedestrian-crossing-scenario}$/;"	l
fig:percemon-architecture	sections/percemon.tex	/^    \\label{fig:percemon-architecture}$/;"	l
fig:percemon-carla-ros	sections/percemon.tex	/^    \\label{fig:percemon-carla-ros}%$/;"	l
fig:percemon-overview	sections/intro.tex	/^  \\label{fig:percemon-overview}$/;"	l
fig:uber-scenario	sections/experiments.tex	/^    \\label{fig:uber-scenario}$/;"	l
gabelaia_combining_2005	bib.bib	/^@article{gabelaia_combining_2005,$/;"	a
gabelaia_computational_2003	bib.bib	/^@inproceedings{gabelaia_computational_2003,$/;"	j
garcia-fernandez_metric_2020	bib.bib	/^@article{garcia-fernandez_metric_2020,$/;"	a
geiger_vision_2013	bib.bib	/^@article{geiger_vision_2013,$/;"	a
gilpin_reasonableness_2018	bib.bib	/^@article{gilpin_reasonableness_2018,$/;"	a
girshick_regionbased_2016	bib.bib	/^@article{girshick_regionbased_2016,$/;"	a
gordon_re3_2018	bib.bib	/^@article{gordon_re3_2018,$/;"	a
haghighi_spatel_2015	bib.bib	/^@inproceedings{haghighi_spatel_2015,$/;"	j
hekmatnejad_formalizing_2021	bib.bib	/^@phdthesis{hekmatnejad_formalizing_2021,$/;"	p
held_learning_2016	bib.bib	/^@inproceedings{held_learning_2016,$/;"	j
hochreiter_long_1997	bib.bib	/^@article{hochreiter_long_1997,$/;"	a
huang_rosrv_2014	bib.bib	/^@inproceedings{huang_rosrv_2014,$/;"	j
jaksic_algebraic_2018	bib.bib	/^@article{jaksic_algebraic_2018,$/;"	a
jaksic_quantitative_2018	bib.bib	/^@article{jaksic_quantitative_2018,$/;"	a
jin_mining_2015	bib.bib	/^@article{jin_mining_2015,$/;"	a
kalman	bib.bib	/^@article{kalman,$/;"	a
kato_autoware_2018	bib.bib	/^@inproceedings{kato_autoware_2018,$/;"	j
kuhn_hungarian_1955	bib.bib	/^@article{kuhn_hungarian_1955,$/;"	a
lee_report_2018	bib.bib	/^@misc{lee_report_2018,$/;"	n
li_efficient_2020	bib.bib	/^@article{li_efficient_2020,$/;"	a
lin_microsoft_2015	bib.bib	/^@article{lin_microsoft_2015,$/;"	a
mahalanobis1936generalized	bib.bib	/^@article{mahalanobis1936generalized,$/;"	a
maler_mitl_2006	bib.bib	/^@inproceedings{maler_mitl_2006,$/;"	j
maler_monitoring_2004	bib.bib	/^@inproceedings{maler_monitoring_2004,$/;"	j
maler_real_2005	bib.bib	/^@inproceedings{maler_real_2005,$/;"	j
maler_synthesizing_2007	bib.bib	/^@inproceedings{maler_synthesizing_2007,$/;"	j
milan_mot16_2016	bib.bib	/^@article{milan_mot16_2016,$/;"	a
nenzi_qualitative_2015	bib.bib	/^@inproceedings{nenzi_qualitative_2015,$/;"	j
nickovic_rtamt_2020	bib.bib	/^@article{nickovic_rtamt_2020,$/;"	a
opendrive_specification	bib.bib	/^@techreport{opendrive_specification,$/;"	t
openscenario_specification	bib.bib	/^@techreport{openscenario_specification,$/;"	t
qin_joint_2019	bib.bib	/^@article{qin_joint_2019,$/;"	a
qin_predictive_2019	bib.bib	/^@inproceedings{qin_predictive_2019,$/;"	j
quigley_ros_2009	bib.bib	/^@inproceedings{quigley_ros_2009,$/;"	j
redmon_yolov3_2018	bib.bib	/^@article{redmon_yolov3_2018,$/;"	a
redmon_you_2016	bib.bib	/^@inproceedings{redmon_you_2016,$/;"	j
ren_faster_2017	bib.bib	/^@article{ren_faster_2017,$/;"	a
ristani_performance_2016	bib.bib	/^@inproceedings{ristani_performance_2016,$/;"	j
rodionova_temporal_2016	bib.bib	/^@inproceedings{rodionova_temporal_2016,$/;"	j
sec:conclusion	main.tex	/^\\label{sec:conclusion}$/;"	l
sec:experiments	main.tex	/^\\label{sec:experiments}$/;"	l
sec:introduction	main.tex	/^\\label{sec:introduction}$/;"	l
sec:percemon	main.tex	/^\\label{sec:percemon}$/;"	l
sec:semantics_for_stql	sections/appendix.tex	/^\\label{sec:semantics_for_stql}$/;"	l
sec:stql	main.tex	/^\\label{sec:stql}$/;"	l
sub:example1	sections/results.tex	/^\\label{sub:example1}$/;"	l
sub:integration_with_carla_and_ros	sections/percemon.tex	/^\\label{sub:integration_with_carla_and_ros}$/;"	l
tab:results	sections/experiments.tex	/^    objects.} \\label{tab:results}$/;"	l
templeton_tesla_2020	bib.bib	/^@misc{templeton_tesla_2020,$/;"	n
thomas_nextgeneration_2014	bib.bib	/^@inproceedings{thomas_nextgeneration_2014,$/;"	j
wojke_simple_2017	bib.bib	/^@inproceedings{wojke_simple_2017,$/;"	j
wu_squeezedet_2017	bib.bib	/^@inproceedings{wu_squeezedet_2017,$/;"	j
wu_tracking_2006	bib.bib	/^@inproceedings{wu_tracking_2006,$/;"	j
yu_bdd100k_2020	bib.bib	/^@article{yu_bdd100k_2020,$/;"	a
yun_recurrent_2019	bib.bib	/^@inproceedings{yun_recurrent_2019,$/;"	j
zapridou_runtime_2020	bib.bib	/^@incollection{zapridou_runtime_2020,$/;"	I
zhang_fairmot_2020	bib.bib	/^@article{zhang_fairmot_2020,$/;"	a
zhang_simple_2020	bib.bib	/^@article{zhang_simple_2020,$/;"	a
zhao_object_2019	bib.bib	/^@article{zhao_object_2019,$/;"	a
zheng2016mars	bib.bib	/^@inproceedings{zheng2016mars,$/;"	j

